Compressive Sensing with Cross-Validation and Stop-Sampling for Sparse Polynomial Chaos Expansions

Compressive sensing is a powerful technique for recovering sparse solutions of underdetermined linear systems, which is often encountered in uncertainty quantification analysis of expensive and high-dimensional physical models. We perform numerical investigations employing several compressive sensing solvers that target the unconstrained LASSO formulation, with a focus on linear systems that arise in the construction of polynomial chaos expansions. With core solvers of l1_ls, SpaRSA, CGIST, FPC_AS, and ADMM, we develop techniques to mitigate overfitting through an automated selection of regularization constant based on cross-validation, and a heuristic strategy to guide the stop-sampling decision. Practical recommendations on parameter settings for these techniques are provided and discussed. The overall method is applied to a series of numerical examples of increasing complexity, including large eddy simulations of supersonic turbulent jet-in-crossflow involving a 24-dimensional input. Through empirical phase-transition diagrams and convergence plots, we illustrate sparse recovery performance under structures induced by polynomial chaos, accuracy and computational tradeoffs between polynomial bases of different degrees, and practicability of conducting compressive sensing for a realistic, high-dimensional physical application. Across test cases studied in this paper, we find ADMM to have demonstrated empirical advantages through consistent lower errors and faster computational times.

==> Makefile <==
SECTIONS = $(wildcard sections/*.tex)
FIGURES_TIKZ = $(shell find figures -type f -name '*.tikz')
FIGURES_TIKZ_PDF = $(FIGURES_TIKZ:%.tikz=%.pdf)
FIGURES_EPS = $(shell find figures -type f -name '*.eps')
FIGURES_EPS_PDF = $(FIGURES_EPS:%.eps=%-eps-converted-to.pdf)
FIGURES_ONLY_PDF = $(shell find figures -type f -name '*.pdf')

all: main.pdf

main.pdf: main.tex $(SECTIONS) $(FIGURES_TIKZ_PDF) $(FIGURES_EPS) \
	$(FIGURES_ONLY_PDF) newcommands_all.tex local.bib
	latexmk -pdf -interaction=nonstopmode main.tex

$(FIGURES_TIKZ_PDF): %.pdf: %.tikz figures/header figures/footer
	cat figures/header $< figures/footer > figures/temp.tex;
	latexmk -pdf -interaction=nonstopmode -jobname=$(basename $@) figures/temp.tex

.PHONY: clean cleanmain cleanall

# You can choose which renegerable files you want to add or exclude below.
clean:
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.glo *.idx *.ilg *.ind *.lof *.log *.lot \
	      *.nav *.out *.ps *.snm *.spl *.toc
	@echo -n "Start cleaning tikz regenerable files..."
	@rm -f $(FIGURES_TIKZ:%.tikz=%.aux)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.bbl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.blg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.brf)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.dvi)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fdb_latexmk)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fls)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.glo)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.idx)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ilg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ind)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lof)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.log)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lot)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.nav)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.out)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ps)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.snm)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.spl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.toc)
	@echo "done."
	cd figures; rm -f temp.tex ;\
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.idx *.ilg *.ind *.log *.out *.ps *.spl *.toc

cleanmain:
	@make clean
	rm -f main.pdf

cleanall:
	@make cleanmain
	@echo "Start cleaning tikz pdf files..."
	@rm -f $(FIGURES_TIKZ_PDF)
	@echo "done."
	@echo "Start cleaning eps pdf files..."
	@rm -f $(FIGURES_EPS_PDF)
	@echo "done."

